GARNET: Reduced-Rank Topology Learning for Robust and Scalable Graph Neural Networks

Graph neural networks (GNNs) have been increasingly deployed in various applications that involve learning on non-Euclidean data. However, recent studies show that GNNs are vulnerable to graph adversarial attacks. Although there are several defense methods to improve GNN robustness by eliminating adversarial components, they may also impair the underlying clean graph structure that contributes to GNN training. In addition, few of those defense models can scale to large graphs due to their high computational complexity and memory usage. In this paper, we propose GARNET, a scalable spectral method to boost the adversarial robustness of GNN models. GARNET first leverages weighted spectral embedding to construct a base graph, which is not only resistant to adversarial attacks but also contains critical (clean) graph structure for GNN training. Next, GARNET further refines the base graph by pruning additional uncritical edges based on probabilistic graphical model. GARNET has been evaluated on various datasets, including a large graph with millions of nodes. Our extensive experiment results show that GARNET achieves adversarial accuracy improvement and runtime speedup over state-of-the-art GNN (defense) models by up to 13.27% and 14.7x, respectively.

==> figure/abla.tex <==
\begin{figure}[ht!]
 %\vspace{-10pt}
    \centering
    \includegraphics[width=\textwidth]{figure/ablation_study.pdf}
    \caption{Comparisons of different kernel combinations in \name on Cora, Pubmed, and Squirrel datasets under Nettack --- We denote the reduced-rank approximation kernel, adaptive filter learning kernel, and adaptive label propagation kernel by Reduced\_Rank, Ada\_Filter, and Ada\_Label\_Prop, respectively. 
    %Note that the red curve is basically \name. 
    \bl{Besides, we choose ProGNN and GPRSVD-CS (GPRGNN + SVD + C\&S) as strong baselines, whose curves on Pubmed are missing due to out-of-memory.}}
    \label{figure:kernels}
    \vspace{-15pt}
\end{figure}

==> figure/graph_rank.tex <==
\begin{figure}[htb]
\begin{center}
	\includegraphics[width=0.6\textwidth]{figure/rank.pdf}
	%\includegraphics[scale=0.5]{figures/GraphZoom_flow1.pdf}
	\caption{Graph rank growth under Metattack. \label{figure:graph_rank}}
\end{center}
%\vspace{-12pt}
\end{figure}

==> figure/rank_compare.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figure/rank_compare_f.pdf}
    \caption{Comparisons of the ranks on input adversarial graph, our reduced-rank graph, and TSVD-based low-rank graph on Cora and Chameleon datasets.}
    \label{figure:rank_comp}
    %\vspace{-5pt}
\end{figure}

==> figure/runtime.tex <==
\begin{figure}[ht]
%\vspace{-5pt}
\begin{center}
\centerline{\includegraphics[width=0.8\columnwidth]{figure/runtime_f.pdf}}
\caption{End-to-end runtime comparison of \name and prior defense methods. We use GPRGNN as the backbone GNN model.}
\label{figure:runtime_comp}
\end{center}
%\vspace{-35pt}
\end{figure}

==> figure/spec_embed_compare.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figure/spec_embed.pdf}
    \caption{GARNET accuracy comparisons of using vanilla spectral embedding and singular components (SC) based spectral embedding in the reduced-rank approximation kernel.}
    \label{figure:spec_comp}
    %\vspace{-5pt}
\end{figure}

==> table/adapt_attack.tex <==
\begin{table}[ht]
  \begin{center}
  %\begin{wraptable}{r}{0.5\linewidth}
    \caption{Averaged accuracy (\%) $\pm$ std under adaptive attacks.}
    %\vspace{8pt}
    \label{table:adapt}
    \begin{adjustbox}{width=0.5\columnwidth,center}
    \begin{tabular}{c|cc|cc}
      %\toprule % <-- Toprule here
      %Dataset & GCN & GPR & GCNSVD & GPRSVD & ProGCN & ProGPR & \name GCN & \name GPR \\
      %$\alpha$ & $\beta$ & $\gamma$ \\
      %\midrule % <-- Midrule here
      \toprule
 &  \multicolumn{2}{c}{Nettack} & \multicolumn{2}{c}{Metattack}\\
\cmidrule(r){2-3} \cmidrule(r){4-5}
Model   &  Ptb. $1$   &  Ptb. $5$  &  Ptb. $10\%$   &  Ptb. $20\%$  \\
\midrule
      Vanilla & $XXX$ & $XXX$ & $XXX$ & $XXX$ \\
      TSVD & $XXX$ & $XXX$ & $XXX$ & $XXX$ \\
      ProGNN & $XXX$ & $XXX$ & $XXX$ & $XXX$ \\
      GNNGuard & $XXX$ & $XXX$ & $XXX$ & $XXX$ \\
      \name & $XXX$ & $XXX$ & $XXX$ & $XXX$ \\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
    \end{adjustbox}
    %\end{wraptable}
  \end{center}
  %\vspace{-10pt}
\end{table}


==> table/hetero.tex <==
\begin{table*}[ht]
  \begin{center}
    \caption{Averaged node classification accuracy (\%) $\pm$ std under non-targeted attack (Metattack) with different perturbation ratio --- We denote the evaluated dataset by its name with the perturbation ratio (e.g., Chameleon-0 means the clean Chameleon graph and Chameleon-10 denotes there are $10\%$ adversarial edges). We bold and underline the first and second highest accuracy, respectively.}
    \vspace{8pt}
    \label{table:hetero}
    \begin{adjustbox}{width=1.6\columnwidth,center}
    \begin{tabular}{c|cccc}
      \toprule % <-- Toprule here
      Dataset & Vanilla-GPRGNN & TSVD-GPRGNN & ProGNN-GPRGNN & \name-GPRGNN\\
      %$\alpha$ & $\beta$ & $\gamma$ \\
      \midrule % <-- Midrule here
      Chameleon-0 & \bl{$\mathbf{61.36} \pm 1.00$} & \bl{$47.29 \pm 1.63$} & $48.39 \pm 0.68$ & $\underline{61.11} \pm 2.46$ \\
      Chameleon-10 & \bl{$\underline{57.55} \pm 1.26$} & \bl{$47.07 \pm 1.21$} & $47.80 \pm 0.91$& $\mathbf{60.96} \pm 1.22$ \\
      Chameleon-20 & \bl{$\underline{53.20} \pm 0.88$} & \bl{$45.12 \pm 1.34$} & $46.69 \pm 0.61$ & $\mathbf{59.96} \pm 0.84$ \\
      \midrule
      %\midrule
      Squirrel-0 & \bl{$\underline{39.51} \pm 1.64$} & \bl{$31.36 \pm 1.87$} & $31.64 \pm 2.87$ & $\mathbf{43.43} \pm 1.14$ \\
      Squirrel-10 & \bl{$\underline{38.27} \pm 0.83$} & \bl{$28.25 \pm 1.66$} & $30.33 \pm 3.29$& $\mathbf{42.62} \pm 1.09$ \\
      Squirrel-20 & \bl{$\underline{35.22} \pm 1.20$} & \bl{$23.91 \pm 1.40$} & $29.36 \pm 3.61$& $\mathbf{41.97} \pm 1.02$ \\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
    \end{adjustbox}
  \end{center}
  \vspace{-18pt}
\end{table*}

==> table/hetero_nettack.tex <==
\begin{table*}[ht]
  \begin{center}
    \caption{Averaged node classification accuracy (\%) $\pm$ std under targeted attack (Nettack) with different perturbation ratio --- We denote the evaluated dataset by its name with the number of perturbations (e.g., Chameleon-0 means the clean Chameleon graph and Chameleon-1 denotes there is $1$ adversarial edge perturbation per target node). We bold and underline the first and second highest accuracy, respectively.}
    \vspace{8pt}
    \label{table:hetero_nettack}
    \begin{adjustbox}{width=1.6\columnwidth,center}
    \begin{tabular}{c|cccc}
      \toprule % <-- Toprule here
      Dataset & Vanilla-GPRGNN & TSVD-GPRGNN & ProGNN-GPRGNN & \name-GPRGNN\\
      %$\alpha$ & $\beta$ & $\gamma$ \\
      \midrule % <-- Midrule here
      Chameleon-0 & \bl{$71.46 \pm 1.92$} & \bl{$62.12 \pm 3.04$} & $58.80 \pm 1.72$& $\underline{72.89} \pm 2.65$ \\
      Chameleon-1 & \bl{$71.02 \pm 1.57$} & \bl{$61.34 \pm 2.93$} & $58.05 \pm 1.90$& $\mathbf{72.68} \pm 1.89$ \\
      Chameleon-2 & \bl{$\underline{70.71} \pm 1.12$} & \bl{$61.09 \pm 2.80$} & $57.44 \pm 1.67$& $\mathbf{72.20} \pm 2.31$ \\
      Chameleon-3 & \bl{$\underline{70.30} \pm 1.28$} & \bl{$60.98 \pm 2.82$} & $57.19 \pm 1.83$& $\mathbf{72.17} \pm 2.07$ \\
      Chameleon-4 & \bl{$69.87 \pm 1.29$} & \bl{$60.85 \pm 3.31$} & $57.44 \pm 1.63$& $\mathbf{72.06} \pm 2.94$ \\
      Chameleon-5 & \bl{$66.26 \pm 1.71$} & \bl{$60.37 \pm 2.86$} & $57.07 \pm 1.82$& $\mathbf{71.83} \pm 2.11$ \\
      \midrule
      %\midrule
      Squirrel-0 & \bl{$\underline{41.36} \pm 2.87$} & \bl{$32.98 \pm 2.36$} & $31.81 \pm 1.72$& $\mathbf{44.91} \pm 1.53$ \\
      Squirrel-1 & \bl{$\underline{41.27} \pm 3.16$} & \bl{$32.63 \pm 0.87$} & $30.54 \pm 2.45$& $\mathbf{43.55} \pm 1.79$ \\
      Squirrel-2 & \bl{$\underline{41.09} \pm 2.14$} & \bl{$32.05 \pm 1.05$} & $30.73 \pm 2.13$& $\mathbf{44.09} \pm 2.35$ \\
      Squirrel-3 & \bl{$\underline{40.98} \pm 2.72$} & \bl{$32.00 \pm 1.66$} & $30.25 \pm 1.98$& $\mathbf{44.18} \pm 2.26$ \\
      Squirrel-4 & \bl{$\underline{40.25} \pm 2.82$} & \bl{$31.45 \pm 1.38$} & $29.09 \pm 2.33$& $\mathbf{43.73} \pm 1.62$ \\
      Squirrel-5 & \bl{$\underline{39.45} \pm 2.36$} & \bl{$31.20 \pm 1.84$} & $27.27 \pm 1.87$& $\mathbf{43.64} \pm 1.53$ \\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
    \end{adjustbox}
  \end{center}
\end{table*}

==> table/rra_algo.tex <==
\SetAlFnt{\large}
\SetAlCapFnt{\large}
\SetAlCapNameFnt{\large}
\IncMargin{1em}
\begin{algorithm}[H]
\LinesNumbered
\KwIn{Adjacency matrix $\mA \in \R^{n \times n}$; kNN graph $k$; sparsification threshold $\delta$}
\KwOut{Reduced-rank adjacency matrix $\tilde{\mA} \in \R^{n \times n}$}
%\SetAlgoLined
 \tcc{Obtain singular components via TSVD}
 $\mU, \mS, \mV^T = truncated\_svd(\mA, rank=50$)\;
 \tcc{Node spectral embedding}
 $\mX = \mU \sqrt{\mS}$\;
 \tcc{Approximate kNN graph construction}
 $\hat{\mA} = kNN\_graph(\mX, k)$\;
 \tcc{Drop edges with node similarity scores lower than $\delta$}
 $\tilde{\mA} = sparsification(\hat{\mA}, \delta)$\;
 \caption{Reduced-rank approximation algorithm (Ours)}
 \label{rra_algor}
\end{algorithm}

==> table/rra_compare.tex <==
\begin{table}[ht!]
  \begin{center}
    \caption{Averaged node classification accuracy (\%) $\pm$ std under targeted attack (Nettack) with different perturbation ratio --- We denote the evaluated dataset by its name with the number of perturbations (e.g., Cora-1 denotes there is $1$ adversarial edge perturbation per target node).}
    \vspace{8pt}
    \label{table:rra}
    \begin{adjustbox}{width=0.5\columnwidth,center}
    \begin{tabular}{c|cc}
      \toprule % <-- Toprule here
      Dataset & GCN-SVD & GCN-RRA \\
      %$\alpha$ & $\beta$ & $\gamma$ \\
      \midrule % <-- Midrule here
      Cora-1 & $70.36 \pm 1.63$ & $\mathbf{79.75} \pm 2.35$  \\
      Cora-2 & $65.66 \pm 2.76$ & $\mathbf{79.69} \pm 1.50$  \\
      Cora-3 & $61.20 \pm 1.93$ & $\mathbf{74.42} \pm 2.06$  \\
      Cora-4 & $57.34 \pm 3.46$ & $\mathbf{60.60} \pm 2.67$  \\
      Cora-5 & $55.30 \pm 2.25$ & $\mathbf{59.04} \pm 2.05$  \\
      \midrule
      Citeseer-1 & $75.23 \pm 2.67$ & $\mathbf{77.30} \pm 2.80$  \\
      Citeseer-2 & $60.15 \pm 2.29$ & $\mathbf{75.23} \pm 2.14$  \\
      Citeseer-3 & $58.89 \pm 5.28$ & $\mathbf{59.84} \pm 3.43$  \\
      Citeseer-4 & $51.74 \pm 7.96$ & $\mathbf{57.94} \pm 5.66$  \\
      Citeseer-5 & $45.07 \pm 2.77$ & $\mathbf{53.18} \pm 3.61$  \\
      \midrule
      %\midrule
      Pubmed-1 & $84.46 \pm 0.28$ & $\mathbf{89.03} \pm 0.68$  \\
      Pubmed-2 & $82.68 \pm 0.46$ & $\mathbf{88.92} \pm 0.45$  \\
      Pubmed-3 & $81.34 \pm 0.68$ & $\mathbf{88.50} \pm 0.45$  \\
      Pubmed-4 & $82.41 \pm 0.54$ & $\mathbf{88.44} \pm 0.64$  \\
      Pubmed-5 & $79.56 \pm 0.48$ & $\mathbf{88.12} \pm 0.86$  \\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
    \end{adjustbox}
  \end{center}
  %\vspace{-16pt}
\end{table}

==> table/runtime.tex <==
\begin{table}[ht]
\centering
\caption{Run time (secs) of each kernel in \name --- We decompose the reduced-rank approximation kernel into truncated SVD (TSVD) and approximate kNN graph construction (AKNN) steps. In addition, we denote the adaptive filter learning kernel and adaptive label propagation kernel by Ada\_Filter, and Ada\_Label\_Prop, respectively.}
\label{table:runtime}
%\renewcommand{\arraystretch}{1.3}
%\scalebox{0.7}{
\begin{tabular}[t]{lccccc}
\toprule
\textbf{Dataset} & TSVD & AKNN  & Ada\_Filter & Ada\_Label\_Prop & Total \\
\midrule
% Cora   &  $0.10$ &  $0.11$ & $1.52$   & $0.04$  & $1.77$  \\
Cora   &  $0.09$ &  $0.10$ & $0.76$   & $0.05$  & $1.00$  \\
% Pubmed   &  $0.31$ &  $0.39$ & $1.48$   & $0.14$  & $2.32$  \\
Pubmed   &  $0.25$ &  $0.72$ & $1.60$   & $0.05$  & $2.62$  \\
% ogbn-arxiv   &  $6.21$ &  $10.31$ & $35.75$   & $0.20$  & $52.47$  \\
% ogbn-products   &  $245.53$ &  $412.63$ & $3002.54$   & $5.02$  & $3665.72$  \\
ogbn-arxiv   &  $6.04$ &  $17.92$ & $40.49$ & $0.23$  & $64.68$  \\
% ogbn-products   &  $358.32$ &  $350.96$ & $2993.52$   & $8.74$  & $3711.54$  \\
% with 4 a6000 and Intel Xeon Silver 4214 CPU @ 2.20GHz (8 cores)
ogbn-products   &  $368.37$ &  $363.32$ & $1139.46$   & $5.21$  & $1876.36$  \\
\bottomrule
\end{tabular}
%}
\end{table}

==> table/svd_algo.tex <==
\SetAlFnt{\large}
\SetAlCapFnt{\large}
\SetAlCapNameFnt{\large}
\IncMargin{1em}
\begin{algorithm}[H]
\LinesNumbered
\KwIn{Adjacency matrix $\mA \in \R^{n \times n}$}
\KwOut{Reduced-rank adjacency matrix $\tilde{\mA} \in \R^{n \times n}$}
%\SetAlgoLined
 $\mU, \mS, \mV^T = truncated\_svd(\mA, rank=50$)\;
 $\tilde{\mA} = \mU \mS \mV^T$\;
 \caption{Truncated SVD based low-rank approximation algorithm}
 \label{svd_algor}
\end{algorithm}
